Sharp Concentration Results for Heavy-Tailed Distributions

We obtain concentration and large deviation for the sums of independent and identically distributed random variables with heavy-tailed distributions. Our concentration results are concerned with random variables whose distributions satisfy $\mathbb{P}(X>t) \leq {\rm e}^{- I(t)}$, where $I: \mathbb{R} \rightarrow \mathbb{R}$ is an increasing function and $I(t)/t \rightarrow \alpha \in [0, \infty)$ as $t \rightarrow \infty$. Our main theorem can not only recover some of the existing results, such as the concentration of the sum of subWeibull random variables, but it can also produce new results for the sum of random variables with heavier tails. We show that the concentration inequalities we obtain are sharp enough to offer large deviation results for the sums of independent random variables as well. Our analyses which are based on standard truncation arguments simplify, unify and generalize the existing results on the concentration and large deviation of heavy-tailed random variables.

==> packages.tex <==
%%% math packeges
\usepackage{amsthm,amsfonts,amsmath,amssymb,dsfont,color, multirow}
\usepackage{commath,enumerate, mathtools}
%\usepackage{hyperref}
%
% \theoremstyle{theorem}
\newtheorem{thm}{\textbf{Theorem}}[]
\newtheorem*{thm*}{\textbf{Theorem}}
\newtheorem{coro}{\textbf{Corollary}}[]
\newtheorem*{coro*}{\textbf{Corollary}}
\newtheorem{lem}{\textbf{Lemma}}
\newtheorem{prop}{\textbf{Proposition}}
\newtheorem{exmp}{\textbf{Example}}
\newtheorem{rem}{\textbf{Remark}}
\newtheorem{defn}{\textbf{Definition}}
%
%%Other packages
% \usepackage[numbers]{natbib}
% \usepackage[square,numbers]{natbib}

% \usepackage{cite}
%\usepackage{balance}
%\usepackage[T1]{fontenc}
%
%% Graphical packages
\usepackage{subcaption, multirow} 
%\usepackage{makecell}
%
%
% Matrix/Vector notation
\newcommand{\mvec}[1]{{\boldsymbol #1}}
\newcommand{\xv}{\mvec{x}}
\newcommand{\cv}{\mvec{c}}
\newcommand{\yv}{\mvec{y}}
\newcommand{\zv}{\mvec{z}}
\newcommand{\diag}[1]{{\rm diag}\intoo{#1}}


% Other symbols
\def\A{\mathcal{A}}
\def\F{\mathcal{F}}
\def\H{\mathcal{H}}
\def\P{\mathcal{P}}
\def\E{\mathcal{E}}
\def\D{\mathcal{D}}
\def\C{\mathcal{C}}
\def\N{\mathcal{N}}
\def\X{\mathcal{X}}
\def\T{\mathcal{T}}
\def\Q{\mathcal{Q}}
\def\rme{{\rm e}}
%
% Probability commands
\newcommand{\p}[2][{}]{\mathbb{P}_{#1} \intoo{#2}}
\newcommand{\e}[2][{}]{\mathbb{E}_{#1} \sbr{#2}}
\newcommand{\expp}[1]{\exp \intoo{#1}}
%
% Norms
\newcommand{\normp}[1]{\norm{#1}_p}
%
% Operators
\newcommand{\define}{\triangleq}
%
%
%% Beamer Setting
%\usepackage[absolute,overlay]{textpos}
%\usepackage{bibentry}
%%\usepackage[sort&compress]{natbib}
%
%% Colored environments
%
%
%\definecolor{Milad}{RGB}{17, 117, 12}
\definecolor{Milad}{RGB}{200, 0, 100}
\definecolor{Reviewer1}{RGB}{42, 0, 208}
\definecolor{Reviewer2}{RGB}{192, 9, 9}
\definecolor{Reviewer3}{RGB}{17, 117, 12}
%
%\newcommand{\milad}[1]{ {\color{Milad} #1 }} 
%\newcommand{\ri}[1]{ {\color{Reviewer1} #1 }} 
%\newcommand{\rii }[1]{ {\color{Reviewer2} #1 }} 
%\newcommand{\riii }[1]{ {\color{Reviewer3} #1 }}

\newcommand{\milad}[1]{  #1 }
\newcommand{\ri}[1]{  #1 }
\newcommand{\rii }[1]{  #1 }
\newcommand{\riii }[1]{  #1 }
